Flexible Mixture Modeling on Constrained Spaces

This paper addresses challenges in flexibly modeling multimodal data that lie on constrained spaces. Such data are commonly found in spatial applications, such as climatology and criminology, where measurements are restricted to a geographical area. Other settings include domains where unsuitable recordings are discarded, such as flow-cytometry measurements. A simple approach to modeling such data is through the use of mixture models, especially nonparametric mixture models. Mixture models, while flexible and theoretically well-understood, are unsuitable for settings involving complicated constraints, leading to difficulties in specifying the component distributions and in evaluating normalization constants. Bayesian inference over the parameters of these models results in posterior distributions that are doubly-intractable. We address this problem via an algorithm based on rejection sampling and data augmentation. We view samples from a truncated distribution as outcomes of a rejection sampling scheme, where proposals are made from a simple mixture model and are rejected if they violate the constraints. Our scheme proceeds by imputing the rejected samples given mixture parameters and then resampling parameters given all samples. We study two modeling approaches: mixtures of truncated Gaussians and truncated mixtures of Gaussians, along with their associated Markov chain Monte Carlo sampling algorithms. We also discuss variations of the models, as well as approximations to improve mixing, reduce computational cost, and lower variance. We present results on simulated data and apply our algorithms to two problems; one involving flow-cytometry data, and the other, crime recorded in the city of Chicago.

==> thrdars_orig.tex <==
\section{Bounding the number of auxiliary variables }
\label{sec:thrdars} 
The MCMC schemes for the two models outlined earlier target the exact
posterior distribution through a data augmentation step that imputes the 
rejected proposals preceding each observation. As described,
this does not {\em a priori} bound the number of rejected proposals. In 
our experiments, we see that as the corresponding MCMC algorithm 
explores parameter space, a cluster will occasionally be produced under 
which the constrained subset $\sub$ has very low probability. This 
could involve a Gaussian whose mean is two or more standard deviations 
away from $\sub$. Producing an accepted proposal from this component 
can require a very large number of rejected proposals. As a consequence, 
the MCMC algorithm will experience a significant slow down, taking a very 
long time to move through an MCMC iteration. This does not just 
increase computational overhead but also affects Markov chain mixing: a 
large number of rejected proposals will increase coupling between 
successive MCMC iterations. Furthermore, a large number of rejected 
samples can swamp out the observations $X$, causing the cluster parameters 
to drift away from the observations and $\sub$, further 
exacerbating the issue. The net effect is longer computation times and 
larger variances in the MCMC estimates. Since MoTG proposes from a 
particular Gaussian component until acceptance (unlike TMoG, which 
picks a new component for each proposal), we expect that this effect is 
worse for MoTG than TMoG. Our experiments confirm this.

To address this, we suggest bounding the maximum number of rejected 
samples per observation. We refer to algorithms with such a bound as 
{\em thresholded samplers}, giving TMoG and MoTG with thresholding. We 
consider different settings of this threshold, including 1, 5, and 50 
rejections per observation. This introduces asymptotic bias into the MCMC 
sampler. 
We will see that introducing bias in this manner reduces the variance in 
both simulation run-times as well as estimates produced, resulting in faster 
and (for reasonable threshold settings) better estimates. Effectively, the threshold 
acts to regularize the proposal distribution $q(x|\theta)$, limiting the amount of probability 
mass it assigns outside $\sub$ by limiting the proportion of rejected samples. 
While it is possible to achieve the same effect through 
priors over $q$ concentrated near $\sub$, this is a simpler and 
more direct approach. \ayu{We should also mention other works that potentially don't introduced bias. Will try to find something for here.}
\ayu{I will mention something about Approximate Bayesian Computation here.}
Section \ref{sec:simstudy} studies the trade-offs involved for different 
threshold settings and the performance of the algorithm in terms of time 
and the predictive likelihood for various simulation studies. 
%We 
%show that thresholding the rejected samples gives comparable result to 
%that of the non-thresholding case, which we call the infinite case from 
%here on out. 
%The thresholding algorithm is a slight tweak of the original
%algorithm as shown in Algorithm \ref{algo:thrshold}. 
%\begin{algorithm}
% \SetAlgoLined
% \KwIn{A sample $x$ and the parameter value $\theta$}
% \KwOut{The set of rejected proposals preceding $x$}
% Initialization\;
% \While{accepted sample $\hat{x}$ has not been drawn or the number of rejected proposals has not exceed threshold $h$}{
% draw $y_i$ independently from $q(.|\theta)$\;
%}
%Discard $\hat{x}$ and treat preceding rejected proposals as $\mathcal{Y}$\;
%\caption{Algorithm to sample from $p(\mathcal{Y}|x, \theta)$}
%\label{algo:thrshold}
%\end{algorithm}

